BuDDI: A Declarative Bloom Language for CALM Programming

Coordination protocols help programmers of distributed systems reason about the effects of transactions on the state of the system, but they're not cheap. Coordination protocols may involve multiple rounds of communication, which can hurt system responsiveness. There exist many efforts in distributed computing for managing the coordination-performance trade-off. More recent is a line of work that characterizes the class of workloads for which coordination is not necessary for consistency: namely, logically monotonic programs. In this paper, we present a case study of logical monotonicity in workloads typical to computational biology. We leverage the Bloom language to write efficient distributed programs, and compare their performance to equivalent programs written in UPC++, a popular language for writing distributed programs. Additionally, we leverage Bloom's analysis tools to identify points-of-coordination, and use our own experience using Bloom to recommend some higher-level abstractions for users without strong distributed computing backgrounds.

==> sections/design.tex <==
% \clearpage

\begin{figure}[t]
    \centering
    \lstinputlisting[style=customc, label={lst:kmerbuddy}, caption={KMER counting in Buddy}]{codes/kmer_c.py}
\end{figure}

\section{Buddy: Python meet SQL}

Why Buddy? Why not just stick with Bloom?
We must show that Buddy is more amenable to analysis and compilation than Bloom.
The kinds of background optimizations we can do with Buddy are not possible or intractable in Bloom.
Open by showing the limitations of Bloom, that should be some motivation. The earlier section should cover some of the benefits (and we'll revisit them later in this section). But it's important to point out key limitations of Bloom to motivate Buddy. Because, after all, we could just write a compiler for Bloom instead.





Buddy is a programming language embedded in Python and SQL, inspired by Bloom.
We build up the language by covering the relevant parts of computation.

\subsection{Dataflow and Data Parallelism}
Everything is a Set. All computation is expressed in either SQL or Set Comprehension.

\begin{lstlisting}[language=Python, caption={Set Comprehension in Python}]
{x for x in iterable}
\end{lstlisting}

\begin{itemize}
    \item Embarrassingly Data Parallel Computation
    \item Side-effect free
\end{itemize}

\subsection{Keep CALM and Merge Lattices}
Pass (+=)

\subsection{Disorderly Execution}
Declarative Algorithms and imperative optimizations.
Stratification
Datalog, Bloom, Daedalus. Functions in Python. Transactios and SAGAs.


First, we discuss the problem of reading and writing data from/to IO devices, such as the disk and network. 

All data is a sequence of bytes. 
Data that arrives continuously is a stream. 

In our view, all computation consists of:
\begin{itemize}
    \item \textbf{IO over Unstructured Data}. For which we use a restricted subset of Python.
    \item \textbf{Queries over Structured Data}. For which we use SQL.
\end{itemize}

\section{Buddy Study: A Static Analysis}

We'll want to show that Buddy is as amenable to static analysis as Bloom (and more amenable to optimizations). We'll specify the syntax and semantics formally with an AST parser, and link to it. Ideally, I'd also like to demonstrate bug detection capabilities in our static analysis. Possibly with rewrite suggestions. We'll talk about how SQL Logical Plans are very amenable to analysis and optimization.

See Listing~\ref{lst:unicast} in the Appendix.

==> sections/overlapdetection.tex <==
\section{Case Study: Genomics Overlap Detection}
This may or may not exist.
